Encoded Spatial Attribute in Multi-Tier Federated Learning

This research presents an Encoded Spatial Multi-Tier Federated Learning approach for a comprehensive evaluation of aggregated models for geospatial data. In the client tier, encoding spatial information is introduced to better predict the target outcome. The research aims to assess the performance of these models across diverse datasets and spatial attributes, highlighting variations in predictive accuracy. Using evaluation metrics such as accuracy, our research reveals insights into the complexities of spatial granularity and the challenges of capturing underlying patterns in the data. We extended the scope of federated learning (FL) by having multi-tier along with the functionality of encoding spatial attributes. Our N-tier FL approach used encoded spatial data to aggregate in different tiers. We obtained multiple models that predicted the different granularities of spatial data. Our findings underscore the need for further research to improve predictive accuracy and model generalization, with potential avenues including incorporating additional features, refining model architectures, and exploring alternative modeling approaches. Our experiments have several tiers representing different levels of spatial aspects. We obtained accuracy of 75.62% and 89.52% for the global model without having to train the model using the data constituted with the designated tier. The research also highlights the importance of the proposed approach in real-time applications.

==> contents/instructions.tex <==
\section{About CAIAC}

The Canadian Artificial Intelligence Association / Association Pour L'Intelligence Artificielle au Canada started out of a workshop in the Spring of 1973 and was originally named as the Canadian Society for Computational Studies of Intelligence/Societé canadienne pour études d'intelligence par ordinateur (CSCSI/SCEIO) and is probably the oldest organized association of its kind. The first formal CSCSI/SCEIO conference happened in 1976. The conference was held biannually for several years until it became an yearly event in 2000. In 2008, CSCSI/SCEIO was officially renamed to CAIAC.

More about our history can be found at \url{https://www.caiac.ca/en/history-of-caiac}. 

\section{Submission Details}
\label{submission}
We invite submissions of both long and short papers. Long papers must be no longer than \textbf{12 pages}, and Short papers must be no longer than \textbf{6 pages}, including references, formatted using the conference template. 

Papers submitted to the conference must contain original work that has not already been published, accepted for publication, or under review by a journal or another conference. Submissions will go through a \textbf{double-blind} review process. Authors are responsible for making sure submissions are anonymized.

A ``Best Paper Award'' and a ``Best Student Paper Award'' will be given at the conference respectively to the authors of each best paper, as judged by the Best Paper Award Selection Committee.

\section{Publication and Registration}
\label{pub}
Since 2020, the conference proceedings are published through PubPub open access\footnote{\url{https://www.pubpub.org/}} and indexed DBLP, ACM, Google Scholar, and other services that access Pubpub publications.

At least one author of each accepted paper is required to attend the conference to present the work. The authors must agree to this requirement prior to submitting their paper for review.

In addition, the corresponding author of each paper, acting on behalf of all of the authors of that paper, must complete and sign a Consent-to-Publish form. The corresponding author signing the copyright form should match the corresponding author marked on the paper.

\section{Figures and Tables}

This simple \LaTeX\xspace template has been tested with \texttt{latex} and with \texttt{pdflatex} commands, directly from the command line or through \texttt{latexmk}. We ask that you place captions below tables and figures as in the examples below.

Pubpub uses a fairly complete \LaTeX\xspace engine that is likely to handle your source files without problems. Please check \url{https://help.pubpub.org/pub/latex-compatibility} if you require specialized packages or non-standard customization.

\begin{figure}[ht]
  \centering
  \ifpdf
    \includegraphics[scale=0.6]{figs/sample_fig.png}
  \else
    \includegraphics[scale=0.6,natwidth=330,natheight=120]{figs/sample_fig.png}
  \fi
  \caption{Captions under figures, please.}
  \label{fig:sample_fig}
\end{figure}

\begin{table}[h]
\begin{tabular}{|l|l|}
\textbf{Header one} & \textbf{Header two} \\ 
\hline
 Some text & More text
\end{tabular}
\vspace{0.2cm}
\caption{Captions under tables, please.}
\label{tab:important}
\end{table}

\section{Using Overleaf}

If you are reading this you have already downloaded the zip file with the template (\textbf{CANAI \conferenceyear\xspace LaTex Template.zip}). All you need to do is to upload it into Overleaf:

\begin{enumerate}
\item Go to \url{overleaf.com}.
\item Click on new project (top left menu).
\item Choose the \textbf{upload project} option.
\item Upload the \textbf{zip file} to Overleaf.
\end{enumerate}

==> tables/dataset_sample.tex <==
% \documentclass{article}
% \usepackage{booktabs}

% \begin{document}

% \begin{table}[ht]
% \centering
% \caption{Sector Values in Canada and Nunavut}
% \label{tab:sector_values}
\resizebox{12cm}{!}{%
\begin{tabular}{ccp{0.35\linewidth}rc}
\toprule
\textbf{REF\_DATE} & \textbf{GEO} & \textbf{Sector} & \textbf{VALUE (Kilotonnes)} & \textbf{Region} \\
\midrule
2009 & Canada & Total, industries and households & 738765.0 & Canada \\
2009 & Canada & Total, industries & 609765.0 & Canada \\
2009 & Canada & Crop and animal production & 62431.0 & Canada \\
2009 & Canada & Forestry and logging & 5331.0 & Canada \\
2009 & Canada & Fishing, hunting and trapping & 648.0 & Canada \\
... & ... & ... & ... & ... \\
2021 & Nunavut & Balancing item: Motor fuels & -307.0 & North \\
2021 & Nunavut & Balancing item: Aviation & 53.0 & North \\
2021 & Nunavut & Balancing item: Synthetic fluorinated gases & 22.0 & North \\
2021 & Nunavut & Balancing item: Non-energy Products from Fuels & -2.0 & North \\
2021 & Nunavut & Balancing item: Other differences & 100.0 & North \\
\bottomrule
\end{tabular}
}
% \end{table}

% \end{document}


==> tables/hierarchy_data.tex <==
\resizebox{6cm}{!}{%
\begin{tabular}{|ccc|c|}
\hline
\multicolumn{1}{|c|}{Country}                  & \multicolumn{1}{c|}{Region}                               & \multicolumn{1}{c|}{Province} & \# of Samples \\ \hline
\multicolumn{1}{|c|}{\multirow{13}{*}{Canada}} & \multicolumn{1}{c|}{\multirow{4}{*}{The Atlantic Region}} & NL                            & 1,288          \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & PE & 1,030           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & NS & 1,519           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & NB & 1,488           \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{2}{*}{Central Canada}} & QC & 1,656           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & ON & 1,657           \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{4}{*}{The West Coast}} & MB & 1,548           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & SK & 1,512           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & AB & 1,621           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & BC & 1,634           \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\multirow{3}{*}{The North}}      & NU & 1,173           \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & NT & 912            \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}                                & YT & 909            \\ \hline
\multicolumn{3}{|c|}{Total}                                                        & \textbf{17,947} \\ \hline
\end{tabular}
}

==> tables/results.tex <==
\resizebox{10cm}{!}{%
\begin{tabular}{l|llll|l}
\hline
                          & Atlantic Region & Central Region & West Region & North Region & Canada   \\ \hline
MSE       & 2764475.79 & 187960267.60 & 124095573.13 & 18978.19 & 12039378800.33 \\ \hline
RMSE & 1662.67    & 13709.86     & 11139.82     & 137.76   & 109724.10      \\ \hline
MAE & 841.90          & 8274.57        & 4760.04     & 86.85        & 25140.87 \\ \hline
R2            & -0.09           & -0.25          & -0.03       & -0.21        & -0.04    \\ \hline
\end{tabular}
}
